Cavity enhancement of V2 centers in 4H-SiC with a fiber-based Fabry-P\'erot microcavity

Silicon vacancy centers in 4H-silicon carbide (SiC) host a long-lived electronic spin and simultaneously possess spin-resolved optical transitions, making them a great candidate for implementing a spin-photon interface. These interfaces are an important building block of quantum networks, which in turn promise to enable secure communication and distributed quantum computing. To achieve this goal, the rate of coherently scattered photons collected from a single emitter needs to be maximized, which can be achieved by interfacing the emitter with an optical cavity. In this work, we integrate V2 centers inside a SiC membrane into a fiber-based Fabry-P\'erot microcavity. We find that SiC lends itself well to membrane fabrication, as evidenced by low surface roughness $\sigma_{\mathrm{RMS}}$ ~ 400 pm, high reproducibility, and consequentially a high cavity finesse F ~ 40 000. At cryogenic temperatures, we observe individual emitters coupling to cavity modes. We confirm their single-emitter character by measuring the second-order autocorrelation function and investigate the Purcell factor by measuring the optical lifetime as a function of the cavity-emitter detuning. We find a 13.3-fold enhancement of photons scattered into the zero-phonon line (ZPL), which could be further increased by using optimized mirror coatings, potentially opening the path towards deterministic spin-photon interaction.

==> texts/contributions.tex <==
List contributions detailed?

